User-Movement-Robust Virtual Reality Through Dual-Beam Reception in mmWave Networks

Utilizing the mmWave band can potentially achieve the high data rate needed for realistic and seamless interaction within a virtual reality (VR) application. To this end, beamforming in both the access point (AP) and head-mounted display (HMD) sides is necessary. The main challenge in this use case is the specific and highly dynamic user movement, which causes beam misalignment, degrading the received signal level and potentially leading to outages. This study examines mmWave-based coordinated multi-point networks for VR applications, where two or multiple APs cooperatively transmit the signals to an HMD for connectivity diversity. Instead of using omnireception, we propose dual-beam reception based on the analog beamforming at the HMD, enhancing the receive beamforming gain towards serving APs while achieving diversity. Evaluation using actual HMD movement data demonstrates the effectiveness of our approach, showcasing a reduction in outage rates of up to 13% compared to quasi-omnidirectional reception with two serving APs, and a 17% decrease compared to steerable single-beam reception with a serving AP. Widening the separation angle between two APs can further reduce outage rates due to head rotation as rotations can still be tracked using the steerable multi-beam, albeit at the expense of received signal levels reduction during the non-outage period.

==> Sec/association.tex <==
\section{User association}
\label{sec_association}

The user association process involves user discovery, serving base station selection and beam training between BS and UE. UE initiates the process by sending a beacon using its wide beam pattern. To make it close to reality, we consider self-blockage by the user's body and antenna placements in the user device, limiting the UE's field of view only towards the user's orientation. The objective of base station selection is to increase the strong spatial receive directions at the UE side, thus, improving the spatial diversity combining gain. 

The beacon is transmitted by the UE using a few URA elements (i.e. $2 \times 2$) in order to generate a wide beam towards the surrounding BSs within the UE's field of view. The beamforming weight vector of this beacon is denoted as $w_{b} \in $  


\subsection{Spatial diversity}


==> Sec/simulation.tex <==
%\section{MIMO System Topology and Connectivity Performance Metrics}
\section{System Topology, Design and Connectivity Performance Metrics}
\label{sec:systemmodel}

\subsection{Coverage on the pitch}


%\textcolor{red}{Mention data rate requirement for an uncompressed 4K or 8K stream}

%Based on our study on the 5G network performance of one of the cellular operators in the UK, the 5G gNodeB inside the stadium is overloaded by the users before and during the match, as shown in Fig.~\ref{fig:5g_network_peformance}. 
Our study on a cellular operator's 5G network performance in Stamford Bridge Chelsea stadium, London, shows that spectators overload the gNodeB in the stadium before and during the match, as shown in Fig.~\ref{fig:5g_network_peformance}.
The gNodeB is placed in one of the stadium rooftop corners. It has three sector antennas where 
Sector-1 partially covers the stadium, 
Sector-2 covers the area outside the stadium, and 
Sector-3 covers the seating areas inside the stadium. 
\textbf{T} indicates the kick-off time. Fig.~\ref{fig:5g_user} and Fig.~\ref{fig:5g_throughput} show the average number of connected users and the average uplink (UL) throughput of all antenna sectors averaged hourly over six different matchdays. The increasing number of connected users and UL throughput can be observed 2 hours before the kick-off time. The peak average connected users and UL throughput of Sector-3 increased to over 12.8 and 16.5 times, respectively, compared to those 6 hours before the match, showing how the network was overloaded during the match. Consequently, the wearable bodycam and sensor application cannot share the same existing public 5G network and compete with the spectators' devices. A private and dedicated network is thus required to serve this use case exclusively.

The wearable bodycam and sensor application require reliable coverage and capacity in the whole pitch area. In this use case, the User Equipment (UE) of each player on the field sends an uplink data stream containing an uncompressed video stream from the bodycam and real-time sensor data to the base stations (BSs). As the players move a lot during the game, the whole pitch area should be covered by the BSs to avoid any zone lacking coverage. As the UEs transmit the uplink streams with a fixed Tx power, the whole pitch area must be covered by uniform channel gain. This could be achieved by strategically deploying the base station antennas inside the stadium.

%To provide coverage on the pitch, t
The BS antennas are placed in the frame of the stadium roof, down-tilted toward the pitch. 
We consider three different antenna placement configurations: C0, C1 and C2, as described in Fig.~\ref{fig:antena_conf}, in which the red squares indicate the location of BS antennas. 
C0 represents the co-located massive MIMO configuration, where all antennas are placed in the center of a stadium side, with half-wavelength spacing between the antennas. 
Meanwhile, C1 and C2 represent the distributed massive MIMO configuration. In C1, the antennas are distributed along one side of the stadium, while in C2, the antennas are distributed along both sides. 
By distributing the antennas throughout the environment, we expect to obtain favourable coverage condition. This condition ensures good reception for the worst locations, achieved when the mean and the minimum Rx level are relatively high~\cite{Andrea2021}. Different shapes of stadiums (e.g. with an oval roof) might require  different BS distribution points.

At the UE side, the antenna can be attached to the player's jersey (e.g. on the shoulder or the upper back part). The antenna design and placement need to consider the shadowing caused by the player's own body part and caused by other players. The typical body movement of players should also be taken into account. 
Nevertheless, the UE antenna design is not the main focus of this paper. For simplicity, we consider using an omnidirectional antenna at the UE. 

%For the UE on the player side, we consider using an omnidirectional antenna. 

\begin{figure}[t]
  \subfloat[Co-located (C0)]{
	\begin{minipage}[b]{0.32\linewidth} 
	   \centering
	   \includegraphics[width=1.0\linewidth]{./Fig/conf_C0.png}
          \label{fig:C0}
	\end{minipage}}%
   \subfloat[Distributed in one side (C1)]{
	\begin{minipage}[b]{0.32\linewidth} 
	   \centering
	   \includegraphics[width=1.0\linewidth]{./Fig/conf_C1.png}
          \label{fig:C1}
	\end{minipage}}%
	\subfloat[Distributed in two sides (C2)]{
	\begin{minipage}[b]{0.32\linewidth}
	   \centering
	   \includegraphics[width=1.0\linewidth]{./Fig/conf_C2.png}
          \label{fig:C2}
	\end{minipage}}
\caption{Massive MIMO antenna placement configurations} 
%\sofie{The red antennas are not that easy to see. Maybe mention that the antennas are red? Can you make them a bit larger?}}
\label{fig:antena_conf}
\end{figure}


We consider $M = 22$ UEs representing 22 players on the pitch and $N$ serving BSs. 
The downlink signal from the \textit{n}-th BS to the \textit{m}-th UE on the field is expressed as:{\begin{equation}
\label{eqn:dl_transmission}
    {{\hat{y}_{mn}^{DL}} =  \sqrt{p_{n}} {\hat{h}_{mn}^{DL}} {x}_{n} + {w}_{m} },
\end{equation}}
where $p_{n}$ is the BS transmit power, $\hat{h}_{mn}^{DL}$ is the downlink channel transfer function between the \textit{n}-th BS and the \textit{m}-th UE, ${x}_{n} $ is the transmitted information by the \textit{n}-th BS, and ${w}_{m}$ is the noise at the \textit{m}-th UE.
Therefore, the total downlink signal from all $N$ base stations received by the \textit{m}-th UE becomes:
\begin{equation}
\label{eqn:sum_dl_transmission}
    {y}_{m}^{DL} = \sum\limits_{n = 1}^{N} {{|\hat{y}_{mn}^{DL}|^2}}.
\end{equation}
%\sofie{This is signal power? I would not call it power, also this is a real signal so maybe avoid using small letter (which was a complex signal in (1))} 
%\rizqi{The complex one uses hat notation}


\subsection{Uplink capacity in massive MIMO}


Since we consider the UE with one antenna transmitting the data stream without precoding, the uplink signal sent by the \textit{m}-th UE and received by the \textit{n}-th BS can be expressed as:
\begin{equation}
\label{eqn:channel}
    {{\hat{y}_{mn}^{UL}} =  \sqrt{p_{m}} {\hat{h}_{mn}^{UL}} {x}_{m} + {w}_{n}},
\end{equation}
where $p_{m}$ is the transmit power of the $m$-th UE, ${\hat{h}_{mn}^{UL}}$ is the uplink channel transfer function between the \textit{m}-th UE and \textit{n}-th BS including the antenna gain at both sides, ${x}_{m}$ 
%$\hat{x}_{m}$ \sofie{why hat?} 
is the transmitted information by the $m$-th UE, and ${w}_{n}$ is the noise at the \textit{n}-th BS. 

\begin{figure}[t]
    \centering
    %\includegraphics[width=0.98\linewidth]{./Fig/stadium_model_setup.png}
    \includegraphics[width=0.88\linewidth]{./Fig/stadium_3dmodel.png}
    \caption{Football stadium 3-D model} 
    \label{fig:stadium_model}
    \vspace{-2mm}
\end{figure}

%The CPU combines all estimated channels between the set of serving BSs with UE$_m$ as $\mathbf{\hat{H}_{m}}$ = $[\mathbf{\hat{h}_{m1}}$, ... , $\mathbf{\hat{h}_{mN}}]$ where $\mathbf{\hat{H}_{m}} \in \mathbb{C}^{M \times N}$.

%The CPU combines all of them to design a precoding vector to transmit information to a UE, creating a cell-free MIMO multi-point scenario. During the channel estimation period, all $L$ serving BSs estimate their channels with UE$_k$, denoted as $\mathbf{\hat{h}_{kl}} \in \mathbb{C}^{L \times 1}$, and the CPU combines all estimated channels between the set of serving BSs with UE$_k$ as $\mathbf{\hat{H}_{k}}$ = $[\mathbf{\hat{h}_{k1}}$, ... , $\mathbf{\hat{h}_{kL}}]$ where $\mathbf{\hat{H}_{k}} \in \mathbb{C}^{L \times L}$.

We consider a cell-free massive MIMO network in which a set of cooperative BSs serves all UEs at the same time-frequency domain~\cite{Ngo_cellfree_2017}. A Central Processing Unit (CPU) coordinating all BSs collects the channel state information from each BS, obtained through the channel estimation process prior to the uplink transmission.  
The uplink channel matrix between all $M$ UEs and $N$ BSs is denoted as $\mathbf{\hat{H}} \in \mathbb{C}^{M \times N}$.
%Maximum Ratio Combining (MRC) and Zero Forcing Combining (ZFC) schemes are considered for the joint processing of $N$ base stations. 
Zero Forcing (ZF) combining scheme is considered for the joint processing of $N$ base stations. 
The combined channel estimation $\mathbf{\hat{H}}$ is then used to determine the combining vector.
%The combining vector of MRC is represented as follows \cite{massivemimobook}:
%\begin{equation}
%\label{eqn:mimo_mr}
%    \mathbf{{V_{}^{MR}} = {\mathbf{\hat{H}_{}}}}  \in \mathbb{C}^{M \times N} ,
%\end{equation}
%while the combining vector of ZFC is represented as follows:
In the ZF scheme, the combining vector is defined as follows~\cite{massivemimobook}:
%\begin{equation}
%\label{eqn:mimo_zf}
%    \mathbf{{V_{}^{ZF}} = \mathbf{\hat{H}_{}} \left( (\mathbf{\hat{H}_{}})^H \mathbf{\hat{H}_{}} \right)^{-1} } \in \mathbb{C}^{M \times N},
%\end{equation}
\begin{equation}
\label{eqn:mimo_zf}
    \mathbf{{V_{}^{ZF}} = \mathbf{\hat{H}_{}} \left( \mathbf{\hat{H}_{}}^T \mathbf{\hat{H}_{}} \right)^{-1} } \in \mathbb{C}^{M \times N},
\end{equation}
in which $\mathbf{V_{}}$ = $[{v_{11}}$, ... , ${v_{MN}}]$ and $\mathbf{\hat{H}^T}$ denotes the nonconjugate transpose of $\mathbf{\hat{H}}$. 

The instantaneous uplink Signal-to-Interference-plus-Noise Ratio (SINR) of transmission from the $m$-th UE to the $n$-th BS after the combining process becomes:

\begin{equation}
\label{eqn:sinr_cfm}
    {{SINR}_{mn}^{UL}} =  
    \frac {{p_{m} |{{v_{mn}^{H}}} {\hat{h}_{mn}}|^{2} }} {
    \sum\limits_{j\neq{m}}^{M} { p_{j} |{{v_{jn}^{H}}} {\hat{h}_{jn}}|^{2}} 
    + {w}_{n}^{2} }. 
\end{equation}
%{\qing{$p_m$ or $p_j$ in the denominator?}}
Therefore, the uplink spectral efficiency per user becomes:
\begin{equation}
\label{eqn:se}
    {SE}_{m}^{UL} = \sum\limits_{n = 1}^{N} {\log_2(1+{SINR}_{mn}^{UL})}.
\end{equation}





\subsection{Simulation environment}
%\label{subsec:antenna}

To recreate an environment as close to reality, we selected Wireless InSite \cite{WirelessInsite}, a 3D ray-tracing simulator widely used in the research community to analyze site-specific radio wave propagation and wireless communication systems. The chosen propagation model is the X3D Ray Model, a full 3D propagation model with a high accuracy achieved through the exact path calculations. %while exploiting GPU acceleration and multithreading. 
For our purpose, we applied a ray spacing of $10^\circ$ with reflections up to the third order and one diffraction per ray.
%, 1 diffraction, and 0 transmissions. 
%All the simulations were performed on a server with 128GB RAM, 24core CPU@4GHz, 1TB SSD and 2x GPU Nvidia A30 24GB. 


We use a 3-D model of Stamford Bridge Chelsea stadium \cite{3dwarehouse_stamford_bridge} in London, UK, as shown in Fig.~\ref{fig:stadium_model}. The model contains over 50.000 polygons with 134 different materials. We then simplified the model by grouping the elements into four main materials: 1) \emph{concrete} with permittivity $\epsilon = 5.31$ F/m, conductivity $\sigma = 0.08987$ S/m and thickness = 30~cm for the main building and tribune, 2) \emph{glass} with $\epsilon = 6.27$ F/m, $\sigma = 0.01915$ S/m, and thickness = 3~mm for the roof covering the tribune, 3) \emph{grass} for the pitch area with the size of 74$\times$109~m$^2$ and 4) \emph{metal} with perfect electric conductor for the frames on the roof and other metal components.    

\begin{figure}[t]
    \centering
    %\includegraphics[scale=0.7]{Fig/5gpatch_wide.png}
    \includegraphics[width=0.6\linewidth]{Fig/5G_patch_pattern.png}
    \caption{Radiation pattern of 5G patch antenna at 3.5 GHz}
    \label{fig:patch}
\end{figure}

Base station antennas are deployed on the stadium frame at 25~m above the pitch, as depicted by the green and yellow boxes in Fig.~\ref{fig:stadium_model}, pointing $60^{\circ}$ downward from the horizon to cover the pitch. 
The distances between antennas in the case of 8, 16, 32, and 64 distributed antennas deployment along one frame are 12.8 m, 6.4 m, 3.2 m and 1.6 m, respectively. 
%The antenna is designed using PCB technology, in particular a 2-layered PCB with a standard FR-4 substrate of the thickness of 1.13mm covered by two layers of copper 0.035mm thick. The patch size is 38.4 mm x 19.5 mm and the ground layer is 85.4 mm x 85.4 mm whose length corresponds to $\lambda/2$ of the operating frequency. The 5G patch antenna pattern is depicted in Fig. \ref{fig:patch}. The simulations were performed with CST Studio and results show a gain of 3.48 dBi gain at the desired frequency and a bandwidth of 250 MHz. 
The base station uses a 5G patch antenna at the 3.5 GHz band designed with CST Studio. The antenna contains a 2-layered PCB with a standard FR-4 substrate of a thickness of 1.13~mm covered by two layers of copper 0.035~mm thick. The patch size is 38.4~mm $\times$ 19.5~mm, and the ground layer is 85.4~mm $\times$ 85.4~mm, whose length corresponds to $\lambda/2$ of the operating frequency. The 5G patch antenna pattern is depicted in Fig.~\ref{fig:patch}, showing a gain of 3.48 dBi at the desired frequency.
On the other side, each UE uses an omnidirectional antenna with a height of 2~m above the pitch.  


\begin{figure*}[t]
    \centering
    %\includegraphics[width=1.0\linewidth]{./Fig/dl_coverage_all_rev.pdf}
    %\caption{Total downlink Rx power for different antenna configurations} 
    \includegraphics[width=0.96\linewidth]{./Fig/dl_coverage_all_channel_gain.pdf}
    \caption{Channel gain for different antenna configurations} 
    \label{fig:coverage_channel_gain}
    \vspace{-2mm}
\end{figure*}


We consider a carrier frequency of 3,510 MHz with 20 MHz bandwidth. The noise figure is assumed to be 7~dB in both BS and UE. The total Tx power of 43 dBm is shared equally among all BS antennas. We consider a downlink transmission from BS to UE in all simulations and assume the uplink-downlink channel reciprocity. 

\subsubsection{Coverage simulation} 
For the coverage analysis, we consider downlink transmission from all BSs to all Rx points on the pitch, distributed in a grid sized 37$\times$54 with a 2~m spacing.
Ray tracing is performed to obtain the downlink channel between each BS and Rx point.
The different numbers of BS antennas: $N = $ 16, 32 and 64, with various configurations: C0, C1 and C2, are simulated.
The total received signal power from all BS antennas in each Rx point is calculated using Eq.~(\ref{eqn:sum_dl_transmission}).  

\subsubsection{Uplink capacity simulation} 
This simulation aims to analyze the uplink capacity of transmission from players on the pitch to base stations. A football game is simulated based on the football players' tracking dataset from~\cite{metrica_football_tracking_dataset}. The dataset contains the actual positions of all players on the pitch during an entire match sampled every 40 ms. The player's movement is only represented by the translation between points since the information about the player's body orientation and rotation are not available on the dataset. 
For the simulation, we sampled the players' positions every 10 s during the first half of a match, resulting in 271-time samples. For each time sample, the static channel state information from $M$ = 22 players to all $N$ base station antennas are acquired to generate $\mathbf{\hat{H}_{}} \in \mathbb{C}^{M \times N \times 271}$.

\subsubsection{Channel aging simulation}
The objective of this simulation is to observe the channel aging impact on uplink capacity. 
%due to the high mobility of the players on the pitch. 
The players' tracking dataset~\cite{metrica_football_tracking_dataset} containing players' positions per 40~ms period are interpolated to generate the players' positions 
%between two consecutive time samples 
per 1~ms. This small-scale movement is simulated to obtain the static channel state information every 1~ms interval during a 40~ms period.



